On the Border Length Minimization Problem (BLMP) on a Square Array

Protein/Peptide microarrays are rapidly gaining momentum in the diagnosis of cancer. High-density and highthroughput peptide arrays are being extensively used to detect tumor biomarkers, examine kinase activity, identify antibodies having low serum titers and locate antibody signatures. Improving the yield of microarray fabrication involves solving a hard combinatorial optimization problem called the Border Length Minimization Problem (BLMP). An important question that remained open for the past seven years is if the BLMP is tractable or not. We settle this open problem by proving that the BLMP is NP-hard. We also present a hierarchical refinement algorithm which can refine any heuristic solution for the BLMP problem. We also prove that the TSP+1-threading heuristic is an O(N)- approximation. The hierarchical refinement solver is available as an opensource code at http://launchpad.net/blm-solve.

==> 0310_recomb_2010_test_cases.txtrecomb.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline 
&&&&&&& \\ 
PROBES & ALGO & LOWER & INIT & HREF & RHREF & PERCENT & TIME \\ 
&&BOUND&COST&&&REFINED& \\ 
\hline \hline 
729 & RAND  &17087 & 26401 & 23970 & 22631 &  14.280\% &  2.83(min) \\ 
729 & SORT  &17087 & 24082 & 22415 & 21649 &  10.103\% &  2.81(min) \\ 
729 & SWM   &17087 & 22267 & 22195 & 22069 &  0.889\% &  2.81(min) \\ 
729 & REPTX &17087 & 21115 & 21107 & 21101 &  0.066\% &  2.81(min) \\ 
729 & EPTX  &17087 & 19733 & 19726 & 19726 &  0.035\% &  2.81(min) \\ 
\hline 
6561 & RAND  &136820 & 243125 & 221090 & 209514 &  13.825\% &  17.55(min) \\ 
6561 & SORT  &136820 & 210326 & 198972 & 191915 &  8.754\% &  17.02(min) \\ 
6561 & SWM   &136820 & 204955 & 204525 & 203412 &  0.753\% &  17.20(min) \\ 
6561 & REPTX &136820 & 185386 & 185362 & 185341 &  0.024\% &  17.16(min) \\ 
6561 & EPTX  &136820 & 168676 & 168623 & 168544 &  0.078\% &  17.15(min) \\ 
\hline 
1024 & RAND  &23480 & 37192 & 35236 & 33046 &  11.148\% &  0.28(sec) \\ 
1024 & SORT  &23480 & 33784 & 32326 & 31026 &  8.164\% &  0.26(sec) \\ 
1024 & SWM   &23480 & 31424 & 31383 & 31323 &  0.321\% &  0.13(sec) \\ 
1024 & QEPX &23480 & 28060 & 28035 & 28028 &  0.114\% &  0.47(sec) \\ 
1024 & REPTX &23480 & 29574 & 29557 & 29546 &  0.095\% &  0.11(sec) \\ 
1024 & EPTX  &23480 & 27591 & 27567 & 27565 &  0.094\% &  0.11(sec) \\ 
\hline 
4096 & RAND  &86818 & 151116 & 143246 & 134485 &  11.005\% &  6.93(sec) \\ 
4096 & SORT  &86818 & 131291 & 127033 & 121742 &  7.273\% &  4.46(sec) \\ 
4096 & SWM   &86818 & 127516 & 127357 & 127092 &  0.333\% &  1.27(sec) \\ 
4096 & QEPX &86818 & 107805 & 107766 & 107702 &  0.096\% &  5.04(sec) \\ 
4096 & REPTX &86818 & 116406 & 116395 & 116376 &  0.026\% &  1.02(sec) \\ 
4096 & EPTX  &86818 & 106471 & 106462 & 106448 &  0.022\% &  1.04(sec) \\ 
\hline 
\end{tabular}


==> approx-algo.tex <==
\section{Algorithms for the BLMP} \label{sec:approx}

\subsection{An $O(N)$-approximation algorithm}

In this section, we will show that a simple version of the algorithm
suggested by Hannenhalli, et al. is actually an $O(N)$-approximation
algorithm. This algorithm can be described as follows. Assume that
the input is the set of strings $S =\{s_1,s_2,\dots,s_{N^2}\}$. The
algorithm first computes a tour $T$ on strings in $S$. Then it
threads the tour $T$ into the grid in row-major order (see Figure
\ref{fig:approx}). The first step can be done by calling the
$\frac{3}{2}$-approximation algorithm for the HTSP suggested by
\cite{1.5-approx-HTSP}.

\begin{figure}
\begin{center}
  \includegraphics[width=2in]{figs/blmp-approx.eps}\\
  \caption{The thick dark line corresponds to an optimal tour on the input strings}\label{fig:approx}
\end{center}
\end{figure}

\begin{lemma}\label{lemma:approx}
$OPT_{HTSP}(S) \leq 2OPT_{BLMP}(S)$.
\end{lemma}

\noindent{\bf Proof:} Let $A$ be an optimal solution for the BLMP on
$S$. Consider the path $P'$ drawn as the thick dark line in Figure
\ref{fig:approx}. Obviously, $Cost(P') \leq Cost(A)=OPT_{BLMP}(S)$.
Let $s_{i_1}$ and $s_{i_{N^2}}$ be the two endpoints of $P'$. Since
the Hamming distance satisfies the triangular inequality,
$\delta(s_{i_1},s_{i_{N^2}}) \leq Cost(P')$. Consider the tour that
starts at $s_{i_1}$, traverses along the path $P'$ to $s_{i_{N^2}}$
and comes back to $s_{i_1}$. Obviously, the cost of the tour is
$Cost(P')+\delta(s_{i_1},s_{i_{N^2}}) \leq 2Cost(P') \leq 2Cost(A)$.
Hence, $OPT_{HTSP}(S) \leq 2OPT_{BLMP}(S)$. $\Box$


\begin{theorem}\label{theorem:approx}
The above algorithm yields an $O(N)$-approximate solution.
\end{theorem}

\noindent{\bf Proof:} First, we see that $Cost(T) \leq
\frac{3}{2}OPT_{HTSP}(S) \leq 3OPT_{BLMP}(S)$. The first inequality
is due to the $\frac{3}{2}$-approximation for the HTSP. The second
inequality is due to Lemma \ref{lemma:approx}. Now let us analyze
the cost of the solution $F$ produced by the algorithm. Consider the
path $P$ drawn as the thick dark line in Figure \ref{fig:approx}.
Obviously, $Cost(P) \leq Cost(T)$. Also, the total cost of the $N$
rows in $F$ is no more than $Cost(P)$. By the triangle inequality,
it is not hard to see that the cost of each column in $F$ is no more
than $Cost(P)$. Therefore, $Cost(F) \leq (N+1)Cost(P) \leq
(N+1)Cost(T)\leq 3(N+1)OPT_{BLMP}(S) = O(N)OPT_{BLMP}(S)$. $\Box$

\input{refine-algo.tex}


==> quad_table.acm.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline 
&&&&&&&&\\
 $N^2$ & LB$^*$ & INIT & EPX & TIME & REF$^*$& QEPX & TIME & REF$^*$\\
&&COST&&(sec)&&&(sec)&\\
&&&&&&&&\\
\hline 
1024 & 23480 & 37192 & 27591 & 0.60 & 25.81\% & 28060 & 0.42 & 24.55\% \\ 
\hline 
1024 & 23427 & 37029 & 27472 & 0.62 & 25.81\% & 28151 & 0.43 & 23.98\% \\ 
\hline 
4096 & 86818 & 151116 & 106471 & 10.70 & 29.54\% & 107805 & 3.05 & 28.66\% \\ 
\hline 
4096 & 86897 & 151176 & 106430 & 10.37 & 29.60\% & 107634 & 3.23 & 28.80\% \\ 
\hline 
16384 & 322129 & 609085 & 410301 & 180.00 & 32.64\% & 411746 & 43.93 & 32.40\% \\ 
\hline 
16384 & - & 608928 & 409625 & 185.88 & 32.73\% & 410902 & 44.70 & 32.52\% \\ 
\hline 
65536 & - & 2447885 & 2447885 & - & 0.00\% & 1563369 & 765.79 & 36.13\% \\ 
\hline 
65536 & - & 2427143 & 2427143 & - & 0.00\% & 1562630 & 774.33 & 35.62\% \\ 
\hline 
\end{tabular}


==> quad_testing_recomb.txt.table.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline 
&&&&&&&&&\\
TEST & PROBES & LOWER & INIT & EPX & TIME & PERCENT & QEPX & TIME & PERCENT  \\
&&BOUND&COST&&(sec)&REFINED&&(sec)&REFINED \\
&&&&&&&&&\\
\hline 
test0 & 1024 & 23480 & 37192 & 27591 & 0.60 & 25.81\% & 28060 & 0.42 & 24.55\% \\ 
\hline 
test1 & 1024 & 23427 & 37029 & 27472 & 0.62 & 25.81\% & 28151 & 0.43 & 23.98\% \\ 
\hline 
test0 & 4096 & 86818 & 151116 & 106471 & 10.70 & 29.54\% & 107805 & 3.05 & 28.66\% \\ 
\hline 
test1 & 4096 & 86897 & 151176 & 106430 & 10.37 & 29.60\% & 107634 & 3.23 & 28.80\% \\ 
\hline 
test0 & 16384 & 322129 & 609085 & 410301 & 180.00 & 32.64\% & 411746 & 43.93 & 32.40\% \\ 
\hline 
test1 & 16384 & - & 608928 & 409625 & 185.88 & 32.73\% & 410902 & 44.70 & 32.52\% \\ 
\hline 
test0 & 65536 & - & 2447885 & 2447885 & - & 0.00\% & 1563369 & 765.79 & 36.13\% \\ 
\hline 
test1 & 65536 & - & 2427143 & 2427143 & - & 0.00\% & 1562630 & 774.33 & 35.62\% \\ 
\hline 
\end{tabular}


==> refine-algo.tex <==
\subsection{A hierarchical refinement algorithm}
\label{sec:hier}
Several heuristics such as the Epitaxial growth have been proposed to solve the BLMP problem earlier. 
However most of these heuristics do not improve the cost monotonically. Local search based 
algorithms are often employed to solve hard combinatorial problems. We now introduce a 
hierarchical refinement algorithm ($HRA$). This refinement technique can be applied 
to any heuristic placement to refine the cost and get a better placement. Let $N$ be the number
of probes in the placement, $d$ a positive integer such that $d^x=N, x\geq 1$ is called the
degree of refinement. The refinement algorithm starts with a given placement, then it divides 
the placement into $s^0_1,s^0_2\ldots s^0_{N/d^2}$ sub-problems with $d^2$ probes per sub-problem. 
Each of these sub-problems is solved optimally -- an optimal permutation among the probes
is found. After this every $d^2$ sub-problems are combined into a new sub-problem 
$s^1_i = \displaystyle\cup_{j=1}^{d^2} s^0_{id^2+j}, 1\leq i \leq N/d^3$. To solve 
$s^1_i$ optimally we identify an optimal permutation among $s^0_{id^2 +j} \in s^1_i,1\leq j \leq d^2$.
This process continues until we are left with no sub-problems to solve. See Figure~\ref{fig:hier_blm}.

We should remark that while solving a sub-problem optimally, we also consider the cost contributed from the 
neighboring sub-problems. This ensures the monotonic improvement in the placement cost. The refinement algorithm 
asymptotically runs in $\Theta(d^2!N)$ time. If $d=O(1)$, the refinement algorithm 
runs in linear time. For small values of $d$, the algorithm performs well in practice. $HRA$ is a
deterministic refinement algorithm. We
further extend this by introducing randomness. The Randomized Hierarchical Refinement Algorithm ($RHRA$)
is similar to the $HRA$ algorithm. $RHRA$ randomly selects a sub-square within the given placement
and applies the $HRA$ technique to the selected sub-square. Similar to local search algorithms, repeating
$RHRA$ algorithm several times improves the placement cost monotonically. We study the performance of both these
algorithms in section~\ref{sec:experiment}.

\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{figs/hier_blm.eps}
\end{center}
\caption{Illustration of the hierarchical refinement algorithm with degree of refinement $3$. This shows
the possible optimal solutions (i.e. permutation among sub-problems) at the top-most and penultimate levels}
\label{fig:hier_blm}
\end{figure}

\subsection{Quad epitaxial algorithm}
\label{sec:quad_epi}
The {\em epitaxial} ($EPX$) placement suggested in~\cite{epitaxial03} places a randomly selected probe at the
center of the array, it continues placing the probes greedily around the locations adjacent to the placed
probes to minimize the cost (i.e. the algorithm almost spends $O(N^2)$ time to place each probe). The 
epitaxial algorithm gives good results for small arrays but for larger arrays the epitaxial algorithm is 
impractical and extremely slow. We propose the Quad Epitaxial ($QEPX$) algorithm as a simple extension to the epitaxial
algorithm. $QEPX$ yields good performance and is very fast compared to the $EPX$ algorithm. The basic
idea behind the $QEPX$ algorithm is to divide the array into four parts, apply $EPX$ algorithm for each
of the four parts and finally find an optimal arrangement among the four parts. In section~\ref{sec:experiment}
we compare the $QEPX$ algorithm with $EPX$ algorithm.

\section{Experimental study} 
\label{sec:experiment}
\subsection{Performance of the $QEPX$ algorithm}
In this section we compare the performance of $QEPX$ algorithm introduced earlier. We use randomly generated 
probe arrays of size $32^2$,$64^2$,$128^2$ and $256^2$. In all of our experimental studies we compute a
{\em lower bound} on the solution by picking the smallest $2N(N-1)$ edges from the complete Hamming distance graph.
Column-$4$(INIT COST) in the table~\ref{table:quad_epx} indicates the placement cost obtained by placing the probes 
in the row major order as given by the input. Column-$5$($8$) indicates the final placement cost obtained by the 
epitaxial (quad) algorithm. As we can see from columns $7$ and $10$, the refinement obtained by the $QEPX$ algorithm 
is very close to the $EPX$ algorithm. On the other hand $QEPX$ runs $3.6X$ faster than the $EPX$ algorithm. As we can 
see from table~\ref{table:quad_epx}, as the chip size increases $EPX$ algorithm becomes very slow. We ran both 
$EPX$ and $QEPX$ algorithms on a chip size of $243\times 243$ with a time limit of $60$ minutes. The $QEPX$ algorithm 
took around $12$ minutes to complete and improved the input placement cost by $36$\%. On the other hand the $EPX$ 
algorithm did not complete the placement. From our experiments we conclude that the $QEPX$ can provide a good placement 
which we can use as an input for refinement/local search algorithms such as $RHRA$. In the next sub-section we provide 
our experimental study of $HRA$ and $RHRA$ algorithms on various placement heuristics.
\begin{table}
\begin{center}
\input{quad_table.tex}
\end{center}
\caption{Comparison between {\em epitaxial} and {\em quad epitaxial} }
\label{table:quad_epx}
\end{table}
\begin{table}
\begin{center}
\input{refined_table.tex}
\end{center}
\caption{Cost refinement for various placement heuristics by applying $HRA$ (hierarchical refinement algorithm) and
$RHRA$ (randomized hierarchical refinement algorithm) with $350$ iterations }
\label{table:refinement}
\end{table}

\subsection{Performance of refinement algorithms}
We have applied our $HRA$, $RHRA$ refining algorithms on the following placement heuristics. 
\begin{itemize}
\item ($RAND$) Random placement: in this placement we just use the order in which the probes
are provided to our algorithm.
\item ($SORT$) Sort placement: in this placement the input probes are sorted lexicographically 
\item ($SWM$) Sliding Window Matching placement is obtained by running the $SWM$~\cite{epitaxial03}
algorithm with parameters $(6,3)$.
\item ($REPX$) Row epitaxial placement is obtained by running the row-epitaxial algorithm with $3$ 
look-ahead rows.
\item ($EPX$) Epitaxial placement is obtained by running the $EPX$ algorithm
\item ($QEPX$) Quad epitaxial placement obtained by our quad-epitaxial algorithm
\end{itemize}
The cost of the placement obtained by running the $HRA$ algorithm exactly once is given in column-5 ($HRA$).
Column-6 ($RHRA$) indicates the placement cost obtained by running our randomized refinement algorithm $RHRA$
for $350$ iterations. From table~\ref{table:refinement} we can see that as initial placement moves closer and
closer towards the lower bound the refinement percentage decreases, which is logical. For test cases with $729$,
$6561$ ($1024$, $4096$) probes we use a refinement degree $d=3$ ($d=2$). Choosing a bigger refinement degree gives
better refinements, however takes more time. Finally we conclude that our refinement algorithms would be very useful
when applied in conjunction with fast initial placement heuristics. A fully function program called {\sf blm-solve}
implementing all our algorithms can be downloaded from the website \url{http://launchpad.net/blm-solve}, the web-site
also has all the supplementary details used in the our experimental study.


==> refined_table.acm.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline 
&&&&&&& \\ 
$N^2$ & ALGO & LB& INIT & HRA & RHRA & & TIME \\ 
&&&COST&&&REF$^*$& \\ 
\hline \hline 
729 & RAND  &17087 & 26401 & 23970 & 22631 &  14.280\% &  2.83(min) \\ 
729 & SORT  &17087 & 24082 & 22415 & 21649 &  10.103\% &  2.81(min) \\ 
729 & SWM   &17087 & 22267 & 22195 & 22069 &  0.889\% &  2.81(min) \\ 
729 & REPTX &17087 & 21115 & 21107 & 21101 &  0.066\% &  2.81(min) \\ 
729 & EPTX  &17087 & 19733 & 19726 & 19726 &  0.035\% &  2.81(min) \\ 
\hline 
6561 & RAND  &136820 & 243125 & 221090 & 209514 &  13.825\% &  17.55(min) \\ 
6561 & SORT  &136820 & 210326 & 198972 & 191915 &  8.754\% &  17.02(min) \\ 
6561 & SWM   &136820 & 204955 & 204525 & 203412 &  0.753\% &  17.20(min) \\ 
6561 & REPTX &136820 & 185386 & 185362 & 185341 &  0.024\% &  17.16(min) \\ 
6561 & EPTX  &136820 & 168676 & 168623 & 168544 &  0.078\% &  17.15(min) \\ 
\hline 
1024 & RAND  &23480 & 37192 & 35236 & 33046 &  11.148\% &  0.28(sec) \\ 
1024 & SORT  &23480 & 33784 & 32326 & 31026 &  8.164\% &  0.26(sec) \\ 
1024 & SWM   &23480 & 31424 & 31383 & 31323 &  0.321\% &  0.13(sec) \\ 
1024 & QEPX &23480 & 28060 & 28035 & 28028 &  0.114\% &  0.47(sec) \\ 
1024 & REPTX &23480 & 29574 & 29557 & 29546 &  0.095\% &  0.11(sec) \\ 
1024 & EPTX  &23480 & 27591 & 27567 & 27565 &  0.094\% &  0.11(sec) \\ 
\hline 
4096 & RAND  &86818 & 151116 & 143246 & 134485 &  11.005\% &  6.93(sec) \\ 
4096 & SORT  &86818 & 131291 & 127033 & 121742 &  7.273\% &  4.46(sec) \\ 
4096 & SWM   &86818 & 127516 & 127357 & 127092 &  0.333\% &  1.27(sec) \\ 
4096 & QEPX &86818 & 107805 & 107766 & 107702 &  0.096\% &  5.04(sec) \\ 
4096 & REPTX &86818 & 116406 & 116395 & 116376 &  0.026\% &  1.02(sec) \\ 
4096 & EPTX  &86818 & 106471 & 106462 & 106448 &  0.022\% &  1.04(sec) \\ 
\hline 
\end{tabular}

